Organized Behavior Classification of Tweet Sets using Supervised Learning Methods

During the 2016 US elections Twitter experienced unprecedented levels of propaganda and fake news through the collaboration of bots and hired persons, the ramifications of which are still being debated. This work proposes an approach to identify the presence of organized behavior in tweets. The Random Forest, Support Vector Machine, and Logistic Regression algorithms are each used to train a model with a data set of 850 records consisting of 299 features extracted from tweets gathered during the 2016 US presidential election. The features represent user and temporal synchronization characteristics to capture coordinated behavior. These models are trained to classify tweet sets among the categories: organic vs organized, political vs non-political, and pro-Trump vs pro-Hillary vs neither. The random forest algorithm performs better with greater than 95% average accuracy and f-measure scores for each category. The most valuable features for classification are identified as user based features, with media use and marking tweets as favorite to be the most dominant.

==> acknowlegment.tex <==
\bf{Acknowledgments}
\label{sec:acknowledgment}

This work is partially supported by the Turkish State Planning Organization (DPT) under the TAM Project, number 2007K120610. The members of the Complex Systems Lab (SosLab) at the Computer Engineering Department of Bogazici University are thanked for their constructive comments and technical support during this work. 

==> algorithm-review.tex <==
\begin{figure*}[t]
	\begin{center}
		\framebox[6.0in]{\begin{minipage}[t]{5.9in}
				\begin{algorithmic}[1]	
					\STATE \textbf{Hashtag} \textit{tracedHashtag}
					\STATE \textbf{Interval} \textit{analysisInterval}
					\STATE \textbf{Integer} \textit{numDays}
					\STATE \textbf{List} \textit{tweets}  
					\STATE \textbf{List} \textit{allUserFeatures} =  $[ ]$
					\STATE \textbf{List} \textit{allTemporalFeatures} =  $[ ]$
					\STATE \textbf{List} \textit{expandedTweets} = $[ ]$
					
					\STATE $tweets \gets getTweets(hashtag=tracedHashtag)$	// Step 1
					\STATE $users \gets  getUsers(tweets)$	
					\FORALL  {$u \in  users$}	
						\STATE $tweets.insert(getTweets(user=u,days=numDays])$ // Step 5
					\ENDFOR
					\FORALL  {$u \in  users$}
						\STATE $userFeatures \gets  extractUserFeatures(u,tracedHashtag, tweets)$
						\STATE $allUserFeatures.insert(<u,userFeatures>)$
					\ENDFOR
					\STATE $timeIntervals \gets  getTimeIntervals(tweets,analysisInterval) $
					\FORALL  {$ti \in  timeIntervals$}
						\STATE $tweetsTI \gets getTweets(tweets,ti)$
						\STATE $temporalFeatures \gets extractTemporalFeatures(tweetsTI)$
						\STATE $allTemporalFeatures.insert(<u,temporalFeatures>))$ 
					\ENDFOR
					\STATE $featureStats \gets computeFeatureStats(allUserFeatures,allTemporalFeatures)$
					\STATE $trainingDataRecord \gets \{allUserFeatures, allTemporalFeatures, featureStats\}$
					\RETURN $trainingDataRecord$ // Step 7
				\end{algorithmic}
		\end{minipage}}
	\end{center}
	\caption[Overview of the feature extraction algorithm.]{Feature extraction algorithm performed on each tweet set of interest.}
	\label{alg:GeneralFeatureExtractionAlgorithm}
	% \vskip
\end{figure*}
